Broadband CPW-based impedance-transformed Josephson parametric amplifier

Quantum-limited Josephson parametric amplifiers play a pivotal role in advancing the field of circuit quantum electrodynamics by enabling the fast and high-fidelity measurement of weak microwave signals. Therefore, it is necessary to develop robust parametric amplifiers with low noise, broad bandwidth, and reduced design complexity for microwave detection. However, current broadband parametric amplifiers either have degraded noise performance or rely on complex designs. Here, we present a device based on the broadband impedance-transformed Josephson parametric amplifier (IMPA) that integrates a horn-like coplanar waveguide (CPW) transmission line, which significantly decreases the design and fabrication complexity, while keeping comparable performance. The device shows an instantaneous bandwidth of 700(200) MHz for 15(20) dB gain with an average saturation power of -110 dBm and near quantum-limited added noise. The operating frequency can be tuned over 1.4 GHz using an external flux bias. We further demonstrate the negligible back-action from our device on a transmon qubit. The amplification performance and simplicity of our device promise its wide adaptation in quantum metrology, quantum communication, and quantum information processing.

==> sections/legacy/3_device.tex <==
\vspace{1em}
\noindent\textbf{Device Description}

\noindent The device layout is shown in Fig. \ref{fig:device}(c). The big features, including the tapered CPW line (green-colored) and the flux line (red-colored), are fabricated with optical lithography and reactive-ion etching (RIE). The plate capacitor (blue-colored) is formed by a layer of AlOx sandwiched by two Al electrodes, and SQUID (yellow-colored) is fabricated with the Dolan-bridge technique\cite{dolan1977offset}. 

We emphasize the simplicity of both the design and the fabrication of the tapered CPW line (green-colored). Though previous research\cite{mutus2014strong} states that a Klopfestein taper formed purely by tapered CPW line is not feasible with the usual photo-lithography technique due to the small CPW gap width, we demonstrate that by loosening the requirements for the maximum reflection loss from -20 dB to -10 dB, we can form a Klopfenstein taper by tapered CPW line with 3 um gap width. In our SIMPA, the 22.5 mm-long tapered CPW line, given by a fixed gap width at 3 um and tapered center-trace width from 7.8 um to 218 um, forms a Klopfenstein taper\cite{pozar2011microwave} and transforms the characteristic impedance $Z_0$ from 50 $\Omega$ to 18 $\Omega$ with -10 dB maximum reflection loss\cite{sp}. The characteristic impedance $Z_0$ and the center trace width along the CPW line are shown in Fig. \ref{fig:device}(a). The parameters of this tapered CPW can be easily calculated by industrial-level CPW line calculators without the need for finite element simulations, and the fabrication can be done with industrial-compatible photo-lithography and RIE.

\\
